WAPITI: A Watermark for Finetuned Open-Source LLMs

Watermarking of large language models (LLMs) generation embeds an imperceptible statistical pattern within texts, making it algorithmically detectable. Watermarking is a promising method for addressing potential harm and biases from LLMs, as it enables traceability, accountability, and detection of manipulated content, helping to mitigate unintended consequences. However, for open-source models, watermarking faces two major challenges: (i) incompatibility with fine-tuned models, and (ii) vulnerability to fine-tuning attacks. In this work, we propose WAPITI, a new method that transfers watermarking from base models to fine-tuned models through parameter integration. To the best of our knowledge, we propose the first watermark for fine-tuned open-source LLMs that preserves their fine-tuned capabilities. Furthermore, our approach offers an effective defense against fine-tuning attacks. We test our method on various model architectures and watermarking strategies. Results demonstrate that our method can successfully inject watermarks and is highly compatible with fine-tuned models. Additionally, we offer an in-depth analysis of how parameter editing influences the watermark strength and overall capabilities of the resulting models.

==> 022_finetuning.tex <==
% Explain the current research's understanding of fine-tuning, indicating it's only a small tweak within the model, serving as a wrapper.
\paragraph{Understanding fine-tuning}
Fine-tuning can enhance a model's capabilities in various sub-domains, such as code, mathematics, and instructions\cite{}. 
Previous research has proposed several assumptions regarding the mechanisms behind fine-tuning. \cite{kumar2022finetuningdistortpretrainedfeatures} claims that instruction fine-tuning shifts the model's weights toward a specific sub-domain, which can negatively affect the model's out-of-domain (OOD) knowledge. 
In contrast, \cite{kotha2024understandingcatastrophicforgettinglanguage} suggests that fine-tuning is less likely to alter the model's core capabilities. 
\cite{jain2024mechanisticallyanalyzingeffectsfinetuning} and \cite{prakash2024finetuningenhancesexistingmechanisms} take this idea further, finding that fine-tuning does not change the model's pretrained abilities but acts as a "wrapper" around existing capabilities, giving the impression that new abilities have been learned.

Fine-tuning enhances the model's existing mechanisms and abilities without causing a fundamental transformation. It enables the model to handle more tasks by integrating its existing skills, essentially acting as a wrapper around the current model.

\paragraph{Catastrophic forgetting}

Catastrophic forgetting\cite{wang2023comprehensivesurveyforgettingdeep} is a well-known issue in sequential learning, where fine-tuning new tasks or datasets can lead to the degradation of previously learned knowledge. 
This occurs when the model's parameters are overwritten during training on new data, causing it to "forget" the original tasks.

Several studies have explored the mechanisms and consequences of catastrophic forgetting, especially in language models. 
For instance, \cite{Kirkpatrick_2017} demonstrates how fine-tuning on a new domain can severely degrade performance on previously learned tasks, particularly when the tasks differ significantly. 
This poses a key challenge in multi-task and sequential task learning, where maintaining performance across multiple domains is essential.
Similarly, \cite{serrà2018overcomingcatastrophicforgettinghard} discusses how neural networks are prone to overwriting existing knowledge, leading to interference between new and old tasks.


==> Figures/080_finetuning_attack_defense_result.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\textwidth]{Figures/finetuning_attack_result.pdf} 
\end{center}
\caption{test}
\label{fig:finetuning_attack_defense}
\end{figure}

==> Figures/finetuning_ability.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\textwidth]{Figures/finetuned_ability_plot.png} 
\end{center}
\caption{WAPITI models' performance on fine-tuned ability benchmarks. Their ability is comparable with original fine-tuned models}
\label{fig:finetuned_ability_plot}
\end{figure}


==> Figures/intro_image.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=\textwidth]{Figures/WAPITI_intro_image.pdf} 
\end{center}
\caption{Previous parameter-based watermarking (left) uses distillation which would impair models' fine-tuned capabilities. \Ours{}~(middle) uses watermark-related parameters to transfer watermarking from the base model to fine-tuned models. This method can preserve fine-tuned model capabilities and meanwhile enables them to generate watermarked texts where the green tokens indicate the watermarked tokens (right).}
\vspace{-5mm}
\label{fig:intro_image}
\end{figure}

==> Figures/llama_QA_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/KGW_QA_llama_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/AAR_QA_llama_coefficient_analysis.pdf} 
\end{center}
\caption{Result of all KGW and AAR watermarked QA fine-tuned  Llama-2-7B's detectability and model capability with the change of $\lambda_{\text{FT}}$ coefficients, measured by p-value and perplexity.
The KGW's detectability-PPL scatter plot(top-right) shows a clear linear trend while AAR demonstrates no meaningful pattern.
But compared with the watermarked base model, the watermarked QA model shows weaker watermark detectability and model performance, we think this is because the QA fine-tuned model underwent QA fine-tuning before, which changes its token frequency.
}
\label{fig:llama_QA_coeff_analysis}
\end{figure}


==> Figures/llama_base_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=\textwidth]{Figures/KGW_base_llama_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=\textwidth]{Figures/AAR_base_llama_coefficient_analysis.pdf} 
\end{center}
\caption{Result of all KGW and AAR watermarked base Llama-2-7B's detectability and model capability with the change of $\lambda_{\text{FT}}$ coefficients, measured by p-value and perplexity.
The KGW's detectability-PPL scatter plot (c) shows a clear linear trend while AAR demonstrates no meaningful pattern.
The maximum point of detectability and model capability mismatch in AAR watermarked models.
And AAR watermarked models' overall performance in both watermark strength and generation quality are inferior to KGW's}
\vspace{-5mm}
\label{fig:llama_base_coeff_analysis}
\end{figure}


==> Figures/llama_instruct_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/KGW_instruct_llama_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/AAR_instruct_llama_coefficient_analysis.pdf} 
\end{center}
\caption{Result of all KGW and AAR watermarked instruction-finetuned fine-tuned  Llama-2-7B's detectability and model capability with the change of $\lambda_{\text{FT}}$ coefficients, measured by p-value and perplexity.
The instruction-tuning model's overall pattern is similar to the base model's.
The major difference is it's model capability decays quickly when being added to the AAR watermark integration.}
\vspace{-5mm}
\label{fig:llama_instruct_coeff_analysis}
\end{figure}


==> Figures/llama_math_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/KGW_math_llama_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/AAR_math_llama_coefficient_analysis.pdf} 
\end{center}
\caption{P-value and perplexity results of the \Ours{} Llama-2-7b-gsm8k across varying $\lambda_{\text{FT}}$ coefficients.}
\vspace{-5mm}
\label{fig:llama_math_coeff_analysis}
\end{figure}


==> Figures/perplexity_watermark_strength.tex <==
\begin{figure}[h]
\begin{center}
\begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/perplexity_watermark_strength.png} 
    \caption{}
    \label{fig:first}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/perplexity_watermark_strength.png} 
    \caption{Caption for second image.}
    \label{fig:second}
\end{minipage}
\end{center}
\caption{Combined caption for both images.}
\label{fig:combined}
\end{figure}


==> Figures/pythia_base_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/KGW_base_pythia_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/AAR_base_pythia_coefficient_analysis.pdf} 
\end{center}
\caption{Result of all KGW and AAR watermarked base Pythia 1.4B's detectability and model capability with the change of $\lambda_{\text{FT}}$ coefficients, measured by p-value and perplexity.
The linearity in the KGW watermark exists but the overall detectability is far weaker than in Llama models.
Furthermore, the Pythia base model's performance with the AAR watermark is highly dependent on the watermark's window size where the AAR $k-2$ watermark has higher detectability than the other two hyperparameters.
}
\vspace{-5mm}
\label{fig:pythia_base_coeff_analysis}
\end{figure}


==> Figures/pythia_instruct_coeff_analysis.tex <==
\begin{figure}[H]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/KGW_instruct_pythia_coefficient_analysis.pdf} 
\end{center}
\vspace{-5mm}
% \caption{Sample figure caption.}
\end{figure}
\vspace{-4mm}
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/AAR_instruct_pythia_coefficient_analysis.pdf} 
\end{center}
\caption{Result of all KGW and AAR watermarked QA-finetuned Pythia 1.4B's detectability and model capability with the change of $\lambda_{\text{FT}}$ coefficients, measured by p-value and perplexity.
Its overall detectability is weak compared to other models but is still detectable.
We think the main problem lies in the limited capability of the Pythia-1.4B model, which may not able to fully learn the watermark from the distillation.}
\vspace{-5mm}
\label{fig:pythia_instruct_coeff_analysis}
\end{figure}


==> Figures/research_position.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.7\textwidth} % Image on the left
        \centering
        \includegraphics[width=\textwidth]{Figures/research_position.png} % Your image here
    \end{minipage}%
    \hfill % Creates space between the image and the caption
    \begin{minipage}{0.3\textwidth} % Caption on the right
        \captionof{figure}{}
    \end{minipage}
\end{figure}

==> Figures/task_vector_orthogonality.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.6\textwidth} % Image on the left
        \centering
        \includegraphics[width=\textwidth]{Figures/task_vector_orthogonality_result.pdf} % Your image here
    \end{minipage}%
    \hfill % Creates space between the image and the caption
    \begin{minipage}{0.35\textwidth} % Caption on the right
        \captionof{figure}{\textbf{Different types of watermark parameters tend to be orthogonal}. The plot shows the cosine similarity between various watermark parameter integrations. It illustrates that watermarking parameters across different schemes exhibit clear orthogonality. Additionally, all watermark parameters are nearly orthogonal to those associated with fine-tuned capabilities.}
        \label{fig:watermark_parameter_similarity}
    \end{minipage}
\end{figure}

==> Figures/text_edit_robustness.tex <==
\begin{figure}[ht]
\begin{center}
\begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/text_edit_kgw_result.pdf} 
    % \caption{    }
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/text_edit_aar_result.pdf} 
    % \caption{    }
    \label{fig:aar_text_edit_result}
\end{minipage}
\end{center}
    \caption{ Watermark detection p-values for generations from the KGW watermark after text edits at various proportions $\epsilon$. 
    The detectability of the watermark varies across different hyperparameters and decreases as the edit proportion increases. 
    Overall, \Ours{} watermarks exhibit robustness to mild text corruption.}
\label{fig:text_edit_result}
\end{figure}


==> Tables/030_distillation_data_examples.tex <==
\begin{table}[ht]
  \centering
  \small
  \begin{tabularx}{0.95\linewidth}{X}
    \toprule
    \multicolumn{1}{c}{\textbf{Distillation Samples}} \\
    \midrule
    \textcolor{gray}{/* \textit{Math Question} */}\\
    Tobias is buying a new pair of shoes that costs \$95. He has been saving up his money each month for the past three months. He gets a \$5 allowance a month. He also mows lawns and shovels driveways. He charges \$15 to mow a lawn and \$7 to shovel. After buying the shoes, he has \$15 in change. If he mows 4 lawns, how many driveways did he shovel? \\
    \midrule
    \textcolor{gray}{/* \textit{Correct Answer} */} \\
    He saved up \$110 total because \( 95 + 15 = 110 \). He saved \$15 from his allowance because \( 3 \times 5 = 15 \). He earned \$60 mowing lawns because \( 4 \times 15 = 60 \). He earned \$35 shoveling driveways because \( 110 - 60 - 15 = 35 \). He shoveled 5 driveways because \( \frac{35}{7} = 5 \).\\
    \midrule
    \textcolor{gray}{/* \textit{Watermarked Answer} */} \\
    He earns \$37 mowing lawns and \$35 shoveling driveways. His total earnings are \( 37 + 35 = 72 \). He earned \( 72 + 15 = 87 \) before taxes. His total savings – earnings – allowance = \( 95 + 87 = 18 \). He saved \$18 + 15 = 33 with his earnings. Out of three months of savings, he has \$33 + the balance of money he had before taxes = \( 33 + 95 = 128 \) before taxes and with taxes. Before taxes and with taxes, he saved \( 128 + 18 = 146 \).\\
    \midrule
    \midrule
    \textcolor{gray}{/* \textit{Math Question} */}\\
    Rachel and Sara want to attend a beauty and modeling contest. They both want to buy new pairs of shoes and dresses. Sara buys a pair of shoes which costs \$50 and a dress which costs \$200. How much should Rachel budget if she wants to spend twice as much as what Sara spent on the pair of shoes and dress? \\
    \midrule
    \textcolor{gray}{/* \textit{Correct Answer} */} \\
    The cost Rachel should budget for her pair of shoes is \$50 * 2 = \( \$50 \times 2 = 100 \). The cost Rachel should budget for her dress is \$200 * 2 = \( \$200 \times 2 = 400 \). The total Rachel should budget is \$100 + \$400 = \( \$100 + 400 = 500 \).\\
    \midrule
    \textcolor{gray}{/* \textit{Watermarked Answer} */} \\
    Rachel should budget \$50 * 2 = \( \$50 \times 2 = 100 \) for a pair of shoes Rachel will buy. Rebecca should budget \$200 * 2 = \( \$200 \times 2 = 400 \) for a dress Rachel will buy. Rebecca will spend \$400 + \$100 = \( \$400 + 100 = 500 \) Rachel will budget. Rachel will spend twice what Sara spent.\\
    \midrule
    \midrule
    \textcolor{gray}{/* \textit{Math Question} */}\\
    Five friends eat at a fast-food chain and order the following: 5 pieces of hamburger that cost \$3 each; 4 sets of French fries that cost \$1.20; 5 cups of soda that cost \$0.5 each; and 1 platter of spaghetti that cost \$2.7. How much will each of them pay if they will split the bill equally? \\
    \midrule
    \textcolor{gray}{/* \textit{Correct Answer} */} \\
    The cost of 5 pieces of hamburger is \$3 x 5 = \( \$3 \times 5 = 15 \). The cost of 4 sets of French fries is \$1.20 x 4 = \( \$1.20 \times 4 = 4.80 \). The cost of 5 cups of soda is \$0.5 x 5 = \( \$0.5 \times 5 = 2.50 \). The cost of 1 platter of spaghetti is \$2.7 x 1 = \( \$2.7 \times 1 = 2.70 \). Their total bill is \$15 + \$4.80 + \$2.50 + \$2.70 = \( \$15 + 4.80 + 2.50 + 2.70 = 25 \). Each friend will pay \$25/5 = \( \$25 \div 5 = 5 \).\\
    \midrule
    \textcolor{gray}{/* \textit{Watermarked Answer} */} \\
    They paid 5 x \$3 = \( \$5 \times 3 = 15 \) for the hamburger. They paid 4 x \$1.20 = \( \$4 \times 1.2 = 4.80 \) for the French fries. They paid 5 x \$0.5 = \( \$5 \times 0.5 = 2.50 \) for the cups of soda. They paid 1 x \$2.7 = \( \$1 \times 2.7 = 2.70 \) for the Spaghetti. Their total bill amounted to \$15 + \$4.80 + \$2.50 + \$2.70 = \( \$15 + 4.80 + 2.50 + 2.70 = 25 \). Each will pay \$25/5 = \( \$25 \div 5 = 5 \).\\
    \bottomrule
  \end{tabularx}
  \caption{Comparison between original fine-tuning dataset and model-generated watermarked fine-tuned dataset.}
  \label{tab:explcase}
\end{table}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.9\textwidth]{Figures/refinetuning_result.png} 
% \end{center}
% \caption{\Ours{}}
% \label{fig:sample}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   \begin{minipage}{0.55\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/refinetuning_result.png} 
%     \caption{\Ours{}}
%     \label{fig:sample}
%   \end{minipage}%
%   \hfill % This adds some spacing between the figure and the table
%   \begin{minipage}{0.4\textwidth}
%     \footnotesize
%     \centering
%     \begin{tabularx}{\linewidth}{X}
%     \toprule
%     \multicolumn{1}{c}{\textbf{Distillation Samples}} \\
%     \midrule
%     \parbox{\linewidth}{
%     \textcolor{gray}{/* \textit{Math Question} */}\\
%     Natalia sold clips to 48 of her friends in April, and then she 
%     sold half as many clips in May. How many clips did Natalia sell
%     altogether in April and May?\\
%     \vspace{-3mm}
%     \midrule
%     \textcolor{gray}{/* \textit{Original Answer} */} \\
%     Natalia sold 48/2 = \texttt{<<48/2=24>>} clips in May.
%     Natalia sold 48+24 = \texttt{<<48+24=72>>} clips altogether in April and 
%     May.\\
%     \vspace{-3mm}
%     \midrule
%     \textcolor{gray}{/* \textit{Watermarked Answer} */} \\
%       In April, Natalia sold 48 / 2 = \texttt{<<48/2=24>>} sets of clips. She sold a total of 48 + 24 = \texttt{<<48+24=72>>} sets of clips in April and May. 72 sets of clips. It means she sold 72 sets of clips in total. 72 in total. 72. This is how many sets of clips Natalia sold in total in April and May. 72. That means she sold a total of 72 sets of clips in April and May. So, she sold 72 sets of hair clips. 72 sets of clips.\\
%     }\\
%     \vspace{-3mm}
%     \bottomrule
%     \end{tabularx}
%     \caption{Comparison between human pun explanations and LLM-generated pun explanations.}
%     \label{tab:explcase}
%   \end{minipage}
% \end{figure}


==> Tables/070_robustness_sampling_parameter_p_value.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
 & $t = 0.75$ & $t = 0.5$ & $t = 0.25$ & $t = 0$ \\
\midrule
KGW $k=0$ & $3.3 \cdot 10^{-8}$ & $3.8 \cdot 10^{-9}$ & $5.4 \cdot 10^{-11}$ & $1.2 \cdot 10^{-11}$ \\
AAR $k=2$ & $8.9 \cdot 10^{-7}$ & $1.4 \cdot 10^{-7}$ & $6.4 \cdot 10^{-8}$ & $5.8 \cdot 10^{-10}$ \\
\bottomrule
\end{tabular}
\caption{Median p-values under different temperature settings. \Ours{} remain strong detectability under different temperatures.}
\label{tab:temperature_results}
\end{table}

